CARDAMOM: A Micro-Dialectal Arabic Speech Dataset for ASR

We present Cardamom, a micro-dialectal Arabic speech dataset designed to support fine-grained evaluation and adaptation of automatic speech recognition (ASR) systems. Community-curated by native speakers familiar with the represented varieties, Cardamom contains approximately 40 hours of transcribed YouTube speech spanning 21 micro-dialects across Egypt, Jordan, Lebanon, Mauritania, Palestine, and Saudi Arabia. Each segment is annotated with one or more operational micro-dialect labels, code-switching information, and utterance-level perceived gender, enabling analysis of sub-country variation that is obscured by conventional country-level labels. We describe the collection and annotation process, motivate the micro-dialect inventory linguistically, and benchmark four multilingual ASR systems in zero-shot and adapted settings. The strongest zero-shot system obtains 43.47% aggregate WER, with particularly high error rates on Mauritanian and Lebanese varieties; adaptation on Cardamom reduces its WER to 35.21%. Audio-based identification experiments further highlight the difficulty of fine-grained micro-dialect recognition: across three training seeds, a dedicated classifier obtains 46.85% accuracy and 31.95% F1. Cardamom provides a resource for studying localized dialectal variation and developing Arabic speech systems with broader regional coverage.

==> Sections/data_analysis.tex <==
\section{Corpus Statistics and Analysis}
\label{sec:corpus_stats}

% \begin{table*}[t!]
% \centering
% \caption{Detailed micro-dialect statistics grouped by country. AVT denotes the average transcript length. U-Wds refers to the total number of unique words, while Avg U-Wds/hr indicates the average number of unique words per hour. Words per second (WPS) and characters per second (CPS) measure average lexical and orthographic density. F\%/M\%: Gender (Female/Male). Totals are aggregated at the country level.}
% \label{tab:micro-dialect-detailed}
% % \scriptsize
% % \setlength{\tabcolsep}{2pt}
% % \resizebox{\textwidth}{!}{%
% \setlength{\tabcolsep}{1.9pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccccccc}
% \hline
% Micro-dialect & Segments & Total Hours & Mean (s) & Min (s) & Max (s) & CS Hours & F\%/M\% & AVT & U-Wds & Avg U-Wds/hr &  WPS & CPS \\
% \hline
% \multicolumn{14}{l}{\textbf{Egypt}} \\
% Cairene & 3793 & 3.388 & 3.216 & 0.164 & 15.446 & 0.208 & 33.3/66.7 & 8.25 & 9922 & 2928.59  & 2.55 & 10.57 \\
% Saidi & 1621 & 1.627 & 3.614 & 0.624 & 57.797 & 0.005 & 37.8/62.2 & 7.94 & 4599 & 2825.81  & 2.18 & 8.77 \\
% Port Saidi & 1078 & 0.978 & 3.265 & 0.223 & 24.539 & 0.034 & 10.9/89.1 & 7.52 & 3145 & 3216.97 &  2.29 & 9.14 \\
% Alexandrian & 831 & 0.746 & 3.230 & 0.580 & 15.630 & 0.020 & 40.5/59.5 & 7.94 & 2953 & 3960.06 &  2.44 & 10.01 \\
% \textbf{\textit{TOTAL}} & \textbf{7110} & \textbf{6.588} & \textbf{3.336} & \textbf{0.164} & \textbf{57.797} & \textbf{0.324} & \textbf{31.8/68.2} & \textbf{8.08} & \textbf{15573} & \textbf{2363.89}  & \textbf{2.41} & \textbf{9.86} \\
% \hline
% \multicolumn{14}{l}{\textbf{Jordan}} \\
% Falahi & 3275 & 4.539 & 4.990 & 0.523 & 33.065 & 0.079 & 18.6/81.4 & 10.69 & 9664 & 2128.96 &  2.12 & 8.33 \\
% Badawi & 2898 & 3.967 & 4.929 & 0.249 & 30.946 & 0.005 & 26.6/73.4 & 8.92 & 7816 & 1970.02 & 1.79 & 6.97 \\
% Madani & 1909 & 2.755 & 5.196 & 0.785 & 35.466 & 0.153 & 38.2/61.8 & 11.82 & 7262 & 2635.51 &  2.27 & 8.88 \\
% \textbf{\textit{TOTAL}} & \textbf{7728} & \textbf{10.806} & \textbf{5.034} & \textbf{0.249} & \textbf{35.466} & \textbf{0.407} & \textbf{26.5/73.5} & \textbf{10.34} & \textbf{18701} & \textbf{1730.69} & \textbf{2.04} & \textbf{7.97} \\
% \hline
% \multicolumn{14}{l}{\textbf{Palestine}} \\
% Falahi & 1564 & 2.720 & 6.260 & 0.446 & 87.218 & 0.021 & 9.0/91.0 & 9.80 & 5532 & 2034.04 & 1.55 & 6.39 \\
% Badawi & 864 & 1.461 & 6.088 & 0.947 & 46.522 & 0.002 & 3.1/96.9 & 8.28 & 3052 & 2088.81 &  1.35 & 5.76 \\
% Madani & 537 & 0.997 & 6.686 & 0.079 & 92.441 & 0.002 & 32.3/67.7 & 8.31 & 2137 & 2142.88 &  1.24 & 5.18 \\
% \textbf{\textit{TOTAL} } & \textbf{2956} & \textbf{5.159} & \textbf{6.283} & \textbf{0.079} & \textbf{92.441} & \textbf{0.031} & \textbf{11.5/88.5} & \textbf{9.07} & \textbf{8581} & \textbf{1663.39} & \textbf{1.43} & \textbf{5.98} \\
% \hline
% \multicolumn{14}{l}{\textbf{Saudi Arabia}} \\
% Hijazi & 1413 & 2.661 & 6.779 & 0.946 & 27.251 & 0.211 & 95.0/5.0 & 15.63 & 5802 & 2180.65 &  2.30 & 9.12 \\
% Southern & 1423 & 2.550 & 6.452 & 0.922 & 63.943 & 0.023 & 40.5/59.5 & 14.84 & 6002 & 2353.34 & 2.29 & 8.70 \\
% Najdi & 1089 & 2.234 & 7.384 & 0.982 & 29.618 & 0.090 & 3.4/96.6 & 14.83 & 5152 & 2306.63 &  2.01 & 7.84 \\
% Eastern & 956 & 2.023 & 7.618 & 0.918 & 51.223 & 0.030 & 17.9/82.1 & 13.26 & 4176 & 2064.37 &  1.70 & 6.66 \\
% Northern & 514 & 1.009 & 7.064 & 1.369 & 15.553 & 0.002 & 0.4/99.6 & 14.87 & 3085 & 3058.74 &  2.10 & 8.74 \\
% \textbf{\textit{TOTAL}} & \textbf{5376} & \textbf{10.425} & \textbf{6.981} & \textbf{0.918} & \textbf{63.943} & \textbf{0.538} & \textbf{39.6/60.4} & \textbf{14.75} & \textbf{17857} & \textbf{1712.90}  & \textbf{2.10} & \textbf{8.23} \\
% \hline§
% \end{tabular}
% }
% % }
% \end{table*}

\begin{table*}[t!]
\centering
\label{tab:micro-dialect-detailed}
% \scriptsize
% \setlength{\tabcolsep}{2pt}
% \resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1.9pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccc}
\hline
Micro-dialect & Segments & Total Hours & Mean (s) & Min (s) & Max (s) & CS Hours & F\%/M\% & AVT & U-Wds & Avg U-Wds/hr & WPS & CPS \\
\hline
\multicolumn{13}{l}{\blue{\textbf{Egypt}}} \\
Cairene & \blue{3,871} & \blue{3.482} & \blue{3.238} & \blue{0.164} & \blue{24.736} & \blue{0.264} & \blue{33.4/66.6} & \blue{8.31} & \blue{11,654} & \blue{3347.22} & \blue{2.55} & \blue{10.88} \\
Saidi & \blue{1,735} & \blue{1.771} & \blue{3.675} & \blue{0.624} & \blue{57.797} & \blue{0.008} & \blue{37.9/62.1} & \blue{8.00} & \blue{5674} & \blue{3,203.63} & \blue{2.13} & \blue{8.91} \\
Port Saidi & \blue{1,124} & \blue{1.021} & \blue{3.269} & \blue{0.223} & \blue{24.539} & \blue{0.039} & \blue{12.2/87.8} & \blue{7.47} & \blue{3,571} & \blue{3,498.42} & \blue{2.27} & \blue{9.28} \\
Alexandrian & \blue{848} & \blue{0.769} & \blue{3.265} & \blue{0.580} & \blue{15.642} & \blue{0.020} & \blue{40.7/59.3} & \blue{8.03} & \blue{3,349} & \blue{4354.29} & \blue{2.44} & \blue{10.31} \\
\blue{\textbf{\textit{TOTAL}}} & \blue{\textbf{7,364}} & \blue{\textbf{6.889}} & \blue{\textbf{3.368}} & \blue{\textbf{0.164}} & \blue{\textbf{57.797}} & \blue{\textbf{0.327}} & \blue{\textbf{32.1/67.9}} & \blue{\textbf{8.13}} & \blue{\textbf{18,805}} & \blue{\textbf{2,729.69}} & \blue{\textbf{2.39}} & \blue{\textbf{10.08}} \\
\hline
\multicolumn{13}{l}{\blue{\textbf{Jordan}}} \\
Falahi & \blue{3,276} & \blue{4.540} & \blue{4.989} & \blue{0.523} & \blue{33.065} & \blue{0.119} & \blue{18.6/81.4} & \blue{10.82} & \blue{10,743} & \blue{2,366.27} & \blue{2.15} & \blue{8.52} \\
Badawi & \blue{2,899} & \blue{3.968} & \blue{4.928} & \blue{0.249} & \blue{30.946} & \blue{0.005} & \blue{26.6/73.4} & \blue{8.97} & \blue{8,057} & \blue{2,030.37} & \blue{1.80} & \blue{7.02} \\
Madani & \blue{1909} & \blue{2.755} & \blue{5.196} & \blue{0.785} & \blue{35.466} & \blue{0.309} & \blue{38.2/61.8} & \blue{11.90} & \blue{7703} & \blue{2,795.56} & \blue{2.28} & \blue{8.99} \\
\blue{\textbf{\textit{TOTAL}}} & \blue{\textbf{7,729}} & \blue{\textbf{10.806}} & \blue{\textbf{5.033}} & \blue{\textbf{0.249}} & \blue{\textbf{35.466}} & \blue{\textbf{0.407}} & \blue{\textbf{26.5/73.5}} & \blue{\textbf{10.43}} & \blue{\textbf{20,504}} & \blue{\textbf{1,897.42}} & \blue{\textbf{2.06}} & \blue{\textbf{8.09}} \\
\hline
\multicolumn{13}{l}{\blue{\textbf{Lebanon}}} \\
\blue{Chamali} & \blue{281} & \blue{0.988} & \blue{12.653} & \blue{1.134} & \blue{31.316} & \blue{0.266} & \blue{9.4/90.6} & \blue{29.69} & \blue{3,212} & \blue{3,252.23} & \blue{2.20} & \blue{9.34} \\
\blue{Jnoubi} & \blue{247} & \blue{0.713} & \blue{10.394} & \blue{0.058} & \blue{30.000} & \blue{0.019} & \blue{16.7/83.3} & \blue{19.33} & \blue{2,253} & \blue{3,159.22} & \blue{1.72} & \blue{6.86} \\
\blue{B'albaki} & \blue{164} & \blue{0.438} & \blue{9.604} & \blue{0.778} & \blue{30.000} & \blue{0.116} & \blue{31.8/68.2} & \blue{19.68} & \blue{1,580} & \blue{3,611.37} & \blue{1.92} & \blue{7.72} \\
\blue{\textbf{\textit{TOTAL}}} & \blue{\textbf{623}} & \blue{\textbf{2.035}} & \blue{\textbf{11.758}} & \blue{\textbf{0.058}} & \blue{\textbf{31.316}} & \blue{\textbf{0.381}} & \blue{\textbf{18.0/82.0}} & \blue{\textbf{24.67}} & \blue{\textbf{58,76}} & \blue{\textbf{2,887.84}} & \blue{\textbf{1.99}} & \blue{\textbf{8.25}} \\
\hline
\multicolumn{13}{l}{\blue{\textbf{Mauritania}}} \\
\blue{Western (Kabla)} & \blue{1,210} & \blue{3.780} & \blue{11.247} & \blue{0.013} & \blue{76.181} & \blue{0.464} & \blue{8.3/91.7} & \blue{25.78} & \blue{9,256} & \blue{2,448.60} & \blue{2.21} & \blue{9.16} \\
\blue{Northern (Sahil)} & \blue{1,205} & \blue{3.809} & \blue{11.380} & \blue{0.013} & \blue{76.181} & \blue{0.470} & \blue{8.1/91.9} & \blue{25.76} & \blue{9,293} & \blue{2,439.56} & \blue{2.16} & \blue{9.02} \\
\blue{Southern (Shark)} & \blue{1,126} & \blue{3.666} & \blue{11.720} & \blue{0.013} & \blue{76.181} & \blue{0.467} & \blue{8.7/91.3} & \blue{26.80} & \blue{9,087} & \blue{2,478.92} & \blue{2.20} & \blue{9.18} \\
\blue{\textbf{\textit{TOTAL}}} & \blue{\textbf{1,314}} & \blue{\textbf{3.998}} & \blue{\textbf{10.953}} & \blue{\textbf{0.013}} & \blue{\textbf{76.181}} & \blue{\textbf{0.473}} & \blue{\textbf{7.7/92.3}} & \blue{\textbf{24.73}} & \blue{\textbf{9,563}} & \blue{\textbf{2,392.07}} & \blue{\textbf{2.16}} & \blue{\textbf{8.96}} \\
\hline
\multicolumn{13}{l}{\blue{\textbf{Palestine}}} \\
Falahi & \blue{1,564} & \blue{2.720} & \blue{6.260} & \blue{0.446} & \blue{87.218} & \blue{0.028} & \blue{9.0/91.0} & \blue{9.91} & \blue{5782} & \blue{2,125.96} & \blue{1.56} & \blue{6.47} \\
Badawi & \blue{864} & \blue{1.461} & \blue{6.088} & \blue{0.947} & \blue{46.522} & \blue{0.001} & \blue{3.1/96.9} & \blue{8.31} & \blue{3,166} & \blue{2,166.83} & \blue{1.36} & \blue{5.81} \\
Madani & \blue{537} & \blue{0.997} & \blue{6.686} & \blue{0.079} & \blue{92.441} & \blue{0.001} & \blue{32.3/67.7} & \blue{8.35} & \blue{2223} & \blue{2229.12} & \blue{1.24} & \blue{5.23} \\
\blue{\textbf{\textit{TOTAL}}} & \blue{\textbf{2,956}} & \blue{\textbf{5.159}} & \blue{\textbf{6.283}} & \blue{\textbf{0.079}} & \blue{\textbf{92.441}} & \blue{\textbf{0.031}} & \blue{\textbf{11.5/88.5}} & \blue{\textbf{9.14}} & \blue{\textbf{9,018}} & \blue{\textbf{1,748.10}} & \blue{\textbf{1.44}} & \blue{\textbf{6.04}} \\
\hline
\multicolumn{13}{l}{\blue{\textbf{Saudi Arabia}}} \\
Southern & \blue{1,423} & \blue{2.550} & \blue{6.452} & \blue{0.922} & \blue{63.943} & \blue{0.088} & \blue{40.5/59.5} & \blue{14.85} & \blue{6,057} & \blue{2,374.90} & \blue{2.30} & \blue{8.71} \\
Hijazi & \blue{1,413} & \blue{2.661} & \blue{6.779} & \blue{0.946} & \blue{27.251} & \blue{0.250} & \blue{95.0/5.0} & \blue{15.65} & \blue{5,937} & \blue{2,231.39} & \blue{2.31} & \blue{9.17} \\
Najdi & \blue{1,089} & \blue{2.234} & \blue{7.384} & \blue{0.982} & \blue{29.618} & \blue{0.156} & \blue{3.4/96.6} & \blue{14.88} & \blue{5,196} & \blue{2,326.32} & \blue{2.01} & \blue{7.87} \\
Eastern & \blue{956} & \blue{2.023} & \blue{7.618} & \blue{0.918} & \blue{51.223} & \blue{0.044} & \blue{17.9/82.1} & \blue{13.26} & \blue{4,183} & \blue{2,067.83} & \blue{1.70} & \blue{6.67} \\
Northern & \blue{514} & \blue{1.009} & \blue{7.064} & \blue{1.369} & \blue{15.553} & \blue{0.003} & \blue{0.4/99.6} & \blue{14.87} & \blue{3,088} & \blue{3,061.71} & \blue{2.10} & \blue{8.74} \\
\blue{\textbf{\textit{TOTAL}}} & \blue{\textbf{5,376}} & \blue{\textbf{10.425}} & \blue{\textbf{6.981}} & \blue{\textbf{0.918}} & \blue{\textbf{63.943}} & \blue{\textbf{0.538}} & \blue{\textbf{39.6/60.4}} & \blue{\textbf{14.77}} & \blue{\textbf{18,113}} & \blue{\textbf{1,737.46}} & \blue{\textbf{2.10}} & \blue{\textbf{8.25}} \\
\hline
\end{tabular}%
}
\caption{\hl{Cations should be below the tables. Please do this for all tables.} Detailed micro-dialect statistics grouped by country. AVT denotes the average transcript length. U-Wds refers to the total number of unique words, while Avg U-Wds/hr indicates the average number of unique words per hour. Words per second (WPS) and characters per second (CPS) measure average lexical and orthographic density. F\%/M\%: Gender (Female/Male). Totals are aggregated at the country level.}
\end{table*}

This section summarizes corpus-level statistics and provides analyses of cross-country and within-country (micro-dialect) variation.

\subsection{Micro-dialect composition and transcript statistics}
Table~\ref{tab:micro-dialect-detailed} reports detailed micro-dialect statistics grouped by country, including segment counts, total hours, average segment duration, CS hours, gender distribution, and transcript-derived metrics (AVT, unique words, and speaking rates).

\textbf{Overall composition.} The dialectal portion of the corpus comprises \blue{25{,}362} segments totaling \blue{$\sim$$40$} hours. At the micro-dialect level, the largest subsets are \blue{Egyptian Cairene (3{,}871 segments; $3.482$ hours), Jordanian Falahi (3{,}276 segments; $4.540$ hours), and Jordanian Badawi (2{,}899 segments; $3.968$ hours).}
% Jordanian Falahi (3{,}275 segments; $4.539$ hours) followed by Egyptian Cairene (3{,}793 segments; $3.388$ hours), and Jordanian Badawi (2{,}898 segments; $3.967$ hours). 
% On the lower-resource end, Saudi Northern ($514$ segments; $1.009$ hours) and Palestinian Madani ($537$ segments; $0.997$ hours) provide smaller but linguistically distinct evaluation conditions.
\blue{On the lower-resource end, Lebanese B'albaki (164 segments; $0.438$ hours), Lebanese Jnoubi (247 segments; $0.713$ hours), and Saudi Northern (514 segments; $1.009$ hours) provide smaller but linguistically distinct evaluation conditions.}

\textbf{Segment duration patterns.} 
\blue{Average duration varies substantially across micro-dialects. Egyptian micro-dialects remain comparatively short (3.238--3.675 seconds), Jordanian micro-dialects occupy a mid-range (4.928--5.196 seconds), and Palestinian and Saudi micro-dialects are longer on average (6.088--7.618 seconds). The newly added Mauritanian and Lebanese subsets introduce the longest average segment durations: Mauritanian varieties range from 11.247 to 11.720 seconds, while Lebanese varieties range from 9.604 to 12.653 seconds. These duration differences likely reflect source-domain effects, especially because the Lebanese and Mauritanian data include a larger share of podcast-style material, where speakers often produce longer, more monologic turns than in everyday conversation. Such variation affects the number of acoustic frames per segment and can influence ASR error patterns and dialect classification decisions.}
% Average duration varies across micro-dialects by more than a factor of two. Egyptian micro-dialects are consistently short (3.216--3.614 seconds), while Palestinian micro-dialects are longer (6.088--6.686 seconds). Saudi micro-dialects show the largest range, with Eastern (7.618 seconds) and Najdi (7.384 seconds) being among the longest, while Southern (6.452 seconds) and Hijazi (6.779 seconds) are comparatively shorter. We attribute part of the longer Saudi segment durations to source-domain effects, as a substantial portion of Saudi data was collected from online podcast-style content in which speakers produce longer, more monologic turns than in everyday conversation. Such duration differences affect the number of acoustic frames per segment and can influence ASR error patterns and dialect classification decisions.

\textbf{Code-switching prevalence.} \blue{CS is highly skewed across micro-dialects, with a small number of varieties accounting for most code-switched speech.\footnote{Such skew is common in naturally collected speech corpora: the presence of CS depends not only on dialect, but also on topic, speaker profile, recording genre, and sociolinguistic exposure to languages such as English or French.} The highest CS amounts are found in Mauritanian Northern (0.470 hours), Mauritanian Southern (0.467 hours), Mauritanian Western (0.464 hours), Jordanian Madani (0.309 hours), Lebanese Chamali (0.266 hours), and Egyptian Cairene (0.264 hours). Appendix~\ref{appendix:codeswitch-examples} provides representative code-switched examples from these and related micro-dialects. In contrast, CS is minimal in Palestinian Badawi and Madani (0.001 hours each), Saudi Northern (0.003 hours), and Jordanian Badawi (0.005 hours).}
% \textbf{Code-switching prevalence.} CS hours are concentrated in a few micro-dialects. The highest CS proportion occurs in Saudi Hijazi (0.211 hours) and Egyptian Cairene (0.208 hours), followed by Jordanian Madani (0.153 hours) and Saudi Najdi (0.090 hours). In contrast, several micro-dialects contain negligible CS (e.g., Jordanian Badawi at 0.005 hours and Palestinian micro-dialects at 0.002--0.021 hours). This implies that CS-aware modeling and evaluation will disproportionately reflect these high-CS subsets.

\textbf{Gender balance.} \blue{Gender distributions are highly micro-dialect dependent. Saudi Hijazi is strongly female-skewed (95.0\% female), whereas the newly added Mauritanian subsets are predominantly male (7.7\%--8.7\% female across the three labels), and Lebanese Chamali is also male-skewed (9.4\% female).\footnote{The female skew in Saudi Hijazi largely reflects the source composition: many Hijazi segments were collected from podcast-style recordings featuring female speakers. In contrast, the male skew in other subsets reflects the speakers and genres available in the corresponding source material.} This imbalance is not only cross-national: gender balance also varies within a single country, e.g., Lebanese B'albaki has 31.8\% female speech compared with 9.4\% for Lebanese Chamali. Such variation may confound cross-dialect comparisons when gender is correlated with channel, register, or topic.}
% \textbf{Gender balance.} Gender distributions are highly micro-dialect dependent. Saudi Hijazi is strongly female-skewed (95.0\% female), while several Bedouin-leaning subsets are predominantly male (e.g., Palestinian Badawi at 3.1\% female and Saudi Najdi at 3.4\% female). Even within the same country, gender balance varies substantially (e.g., Jordanian Madani at 38.2\% female versus Falahi at 18.6\% female), which can confound cross-dialect comparisons if gender is correlated with channel, register, or topic.

\textbf{Lexical and transcript-derived statistics.} \blue{The highest average transcript length (AVT) values are observed in the Lebanese and Mauritanian subsets, led by Lebanese Chamali (29.69), Mauritanian Southern (26.80), Mauritanian Western (25.78), and Mauritanian Northern (25.76). These differences likely reflect variation in source genre and segmentation granularity, since podcast-style or conversational recordings tend to yield longer transcripts than short-form clips or more tightly segmented speech. Unique-word rates (Avg U-Wds/hr) show similarly strong within-country variation. In Egypt, Alexandrian has the highest rate (4{,}354.29 words/hour), followed by Port Saidi (3{,}498.42) and Saidi (3{,}203.63). In Lebanon, B'albaki has the highest rate (3{,}611.37 words/hour), followed by Chamali (3{,}252.23) and Jnoubi (3{,}159.22). These differences may affect vocabulary coverage and out-of-vocabulary behavior in downstream ASR and dialect modeling experiments.}

% \textbf{Lexical and transcript-derived statistics.} Saudi micro-dialects exhibit the highest AVT values (14.87 for Northern, 15.63 for Hijazi, 14.84 for Southern), suggesting a higher lexical variety per segment. Unique-word rates (Avg U-Wds/hr) highlight strong within-country variation. In Egypt, Alexandrian has the highest rate (3{,}960 words/hour) followed by Port Saidi (3{,}216 words/hour), while Saidi is lower (2{,}825 words/hour). In Jordan, Madani shows a higher unique-word rate (2{,}635 words/hour) than Falahi (2{,}128 words/hour) and Badawi (1{,}970 words/hour). These differences can affect vocabulary coverage and out-of-vocabulary behavior in ASR and dialect modeling.

\textbf{Speech rate comparisons.} \blue{Using words-per-second (WPS) and characters-per-second (CPS) as coarse proxies for speaking rate, the Egyptian and some Saudi varieties exhibit the fastest speech, while Palestinian and Lebanese subsets are comparatively slower. These differences may influence ASR behavior, particularly insertion and deletion errors, and should be considered in cross-dialect evaluation.


% the fastest micro-dialects are Egyptian Cairene (WPS 2.55; CPS 10.88), Egyptian Alexandrian (WPS 2.44; CPS 10.31), Saudi Hijazi (WPS 2.31; CPS 9.17), and Saudi Southern (WPS 2.30; CPS 8.71). The slowest subsets are Palestinian Madani (WPS 1.24; CPS 5.23), Palestinian Badawi (WPS 1.36; CPS 5.81), and Lebanese Jnoubi (WPS 1.72; CPS 6.86), reflecting both longer segment durations and lower token rates. These rate differences can impact ASR decoding (e.g., insertion/deletion patterns) and should be controlled for in cross-micro-dialect benchmarking.}

\textbf{Domain and sampling bias.} The above distributions and derived metrics are influenced by the domain of the underlying YouTube sources (e.g., interviews vs. vlogs, topic, recording conditions, and conversational formality) and by the segmentation strategy. Consequently, differences in duration, CS prevalence, lexical statistics, and rate-related metrics may partially reflect domain composition rather than purely linguistic variation.




% \subsection{Quantifying the Dialectal Continuum}

% \noindent To investigate the linguistic boundaries between varieties, we analyze the frequency of multi-label assignments. This serves as a proxy for dialect leveling and the existence of a linguistic continuum.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/combined_continuum_final.pdf}
%     \caption{Cross-micro-dialect overlap based on multi-label assignments (co-occurrence matrices) across the four countries.}
%     \label{fig:combined_continuum}
% \end{figure*}

% \noindent\textbf{Regional variation and contiguity.} As shown in Figure~\ref{fig:combined_continuum}, the density of the co-occurrence matrices varies significantly by region. Jordan exhibits the highest overlap (4.34\%), centered on the Madani--Falahi (171 segments) and Badawi--Falahi (177 segments) intersections. This provides empirical support for the discussion in Section~6.1.1 regarding the stabilization of an urban koin\'e in Amman, where features from rural and northern varieties are frequently merged.

% \noindent\textbf{Prestige hubs in Egypt.} The Egypt matrix (2.90\% overlap) reveals a star-like topology where the Cairene variety acts as the primary hub, overlapping with Alexandrian (129) and Port Saidi (67). This pattern is consistent with a prestige-driven continuum in which regional speakers adopt Cairene features while maintaining their base variety.

% \noindent\textbf{Annotator bias and category discreteness.} We observe substantially lower overlap in Palestine (0.30\%) and Saudi Arabia (0.35\%). While the Saudi results align with the geographic isolation of its regions (Section~6.3), the Palestinian results may reflect annotator behavior. Despite the geographical contiguity of Palestinian varieties, sharp phonological markers (e.g., \textit{qaf} and \textit{kaaf} realizations) may encourage annotators to favor a single, discrete label over multi-label assignment. This suggests that while a continuum exists in practice, perceived sociolinguistic boundaries in these regions remain highly salient to native speakers.



% --- Qualitative Analysis Section ---

% \subsection{Distribution of Emotions}
% \textcolor{blue}{Bashar.. Show the distribution of emotions per country.}





\subsection{Quantitative Inter-category Overlap}
\label{subsec:quant_overlap}

To move beyond aggregate statistics, we examine the fluid boundaries between linguistic varieties by analyzing the frequency and nature of multi-label assignments. These overlaps serve as an empirical proxy for dialectal convergence and the existence of a linguistic continuum in spontaneous speech.

\blue{The density of the dialectal continuum varies significantly across the sampled regions. As shown in Table~\ref{tab:dialect_intersections}, the largest overlap occurs in \textbf{Mauritania}, where the three Hassaniya-oriented regional labels are highly co-assigned: \textbf{Northern--Southern} (1{,}114), \textbf{Southern--Western} (1{,}112), and \textbf{Northern--Western} (1{,}110). However, this pattern should be interpreted with caution. Because Mauritanian Arabic is highly low-resource, micro-dialect-specific source material was difficult to obtain. Much of the available data instead comes from mainstream or broadly shared Hassaniya speech, such as public or media-style recordings, whose utterances are likely understood and used across regions. As a result, many Mauritanian segments were labeled with multiple regional micro-dialects rather than assigned to a single sharply localized variety. The high overlap therefore reflects both genuine dialectal continuity and the scarcity of clearly micro-dialect-specific data.}

\blue{Beyond Mauritania, \textbf{Jordan} exhibits the most substantial overlap, with near-parity between \textbf{Badawi--Falahi} (178) and \textbf{Falahi--Madani} (171), while \textbf{Badawi--Madani} remains much lower (23). This pattern supports the interpretation of Falahi as a central bridging variety between Bedouin and urban speech in the Jordanian sub-corpus. In contrast, the \textbf{Egypt} sub-corpus reveals a more hub-and-spoke topology centered on \textbf{Cairene}, which shares substantial overlap with coastal varieties such as \textbf{Alexandrian} (130) and \textbf{Port Saidi} (67), while links involving Saidi and other regional-to-regional intersections remain sparse (2--10).}

\blue{At the same time, other micro-dialects within the same country show strong separation from one another. This is most evident in \textbf{Saudi Arabia}, where most pairwise overlaps are minimal (e.g., \textbf{Eastern--Southern} (1)). These low-overlap cases suggest that, despite some fluid boundaries, many within-country micro-dialect labels remain relatively well separated in the corpus.}

% The density of the dialectal continuum varies significantly between the sampled regions. As shown in Table~\ref{tab:dialect_intersections}, \textbf{Jordan} exhibits the most substantial overlap, with the near-parity of \textbf{Falahi--Badawi} (177) and \textbf{Falahi--Madani} (171) intersections. This suggests that in the Jordanian context, rural varieties function as a central linguistic bridge. In contrast, the \textbf{Egypt} sub-corpus reveals a hub-and-spoke topology centered on \textbf{Cairene}, which shares significant segments with coastal varieties such as \textbf{Alexandrian} (129) and \textbf{Port Saidi} (67), while regional-to-regional intersections remain sparse.

\blue{To ground these overlaps qualitatively, Table~\ref{tab:multi_label_examples} provides representative multi-label segments from regions with different overlap profiles. In \textbf{Jordan}, examples such as \<يلا بخاطرك> (Badawi, Falahi) and \<اه والله مزبوط> (Falahi, Madani) illustrate how broadly shared lexical items and discourse markers can blur perceived boundaries between rural, Bedouin, and urban varieties. In \textbf{Egypt}, \<استنى يابا> (Alexandrian, Port Saidi) and \<فلوس باباكي متلزمناش> (Alexandrian, Cairene) show that overlap is often concentrated around common everyday expressions, while the stronger Alexandrian--Cairene and Cairene--Port Saidi intersections are consistent with Cairene functioning as a central metropolitan variety. In \textbf{Saudi Arabia}, overlap is much rarer, but examples such as \<تماما ينطبق نفس الشي على الرجال> (Hijazi, Najdi) indicate that shared formal or broadly intelligible phrasing can still lead to co-labeling. Overall, these examples suggest that multi-label assignments arise from a mixture of shared lexical material, broadly intelligible discourse patterns, and region-specific degrees of dialectal separation.}

% To ground these overlaps qualitatively, Table~\ref{tab:multi_label_examples} provides representative multi-label segments. For instance, the Jordanian segment \<يلا بخاطرك> (Badawi, Falahi) and \<اه والله مزبوط> (Falahi, Madani) illustrate cases where broadly shared lexical terms and discourse markers reduce perceived boundaries between rural and urban varieties. In Egypt, \<استنى يابا> (Alexandrian, Cairene, Port Saidi) exemplifies an utterance that is compatible with multiple coastal and metropolitan varieties, whereas \<فلوس باباكي متلزمناش> (Alexandrian, Cairene) reflects a more focused overlap consistent with Cairene acting as a prestige hub. Saudi overlap is rare but still observable (e.g., \<فشهر واحد جاتنا اربعة حالات> as Hijazi, Najdi), while in Palestine, overlap appears limited despite geographic contiguity, suggesting stronger perceived boundaries in annotation practice.

Finally, we note that the observed overlap counts can be influenced by \textit{(i)} the domain of the underlying audio clips (e.g., interviews, vlogs, podcasts) and topic/register, and \textit{(ii)} annotator decision strategies. In particular, some annotators may implicitly treat labeling as single-label even when multi-labeling is permitted, which may contribute to the very low overlap observed for Palestinian varieties.

\begin{table}[t!]
\label{tab:dialect_intersections}
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}

\begin{tabular}{@{}lllr@{}}
\toprule
\rowcolor{gray!15}
\textbf{Region} & \textbf{Dialect A} & \textbf{Dialect B} & \textbf{Overlap Count} \\ 
\midrule

\rowcolor{green!6}
\textbf{Egypt} & Alexandrian & Cairene & 130 \\
\rowcolor{green!6}
               & Alexandrian & Port Saidi & 10 \\
\rowcolor{green!6}
               & Alexandrian & Saidi & 3 \\
\rowcolor{green!6}
               & Cairene & Port Saidi & 67 \\
\rowcolor{green!6}
               & Cairene & Saidi & 9 \\
\rowcolor{green!6}
               & Port Saidi & Saidi & 2 \\ 
\cmidrule(l){2-4}

\rowcolor{blue!6}
\textbf{Jordan} & Badawi & Falahi & 178 \\
\rowcolor{blue!6}
                & Badawi & Madani & 23 \\
\rowcolor{blue!6}
                & Falahi & Madani & 171 \\ 
\cmidrule(l){2-4}

\rowcolor{purple!6}
\textbf{Lebanon} & B'albaki & Chamali & 31 \\
\rowcolor{purple!6}
                 & B'albaki & Jnoubi & 30 \\
\rowcolor{purple!6}
                 & Chamali & Jnoubi & 32 \\ 
\cmidrule(l){2-4}

\rowcolor{cyan!7}
\textbf{Mauritania} & Northern  & Southern  & 1114 \\
\rowcolor{cyan!7}
                    & Northern  & Western  & 1110 \\
\rowcolor{cyan!7}
                    & Southern  & Western & 1112 \\ 
\cmidrule(l){2-4}

\rowcolor{red!5}
\textbf{Palestine} & Badawi & Madani & 6 \\
\rowcolor{red!5}
                   & Falahi & Madani & 3 \\ 
\cmidrule(l){2-4}

\rowcolor{yellow!8}
\textbf{Saudi} & Eastern & Najdi & 3 \\
\rowcolor{yellow!8}
               & Eastern & Southern & 1 \\
\rowcolor{yellow!8}
               & Hijazi & Najdi & 14 \\
\rowcolor{yellow!8}
               & Northern & Southern & 1 \\ 
\bottomrule

\end{tabular}
\caption{Primary micro-dialectal intersections by region, reflecting the most fluid linguistic boundaries in the corpus.}
\end{table}

% \begin{table}[h]
% \caption{Multi-label annotation density across the MicroDA sub-corpora.}
% \label{tab:multilabel_stats}
% \centering
% \begin{tabular}{@{}lrrr@{}}
% \toprule
% \textbf{Region} & \textbf{Total Segments} & \textbf{Multi-label Count} & \textbf{Multi-label } \\ \midrule
% Jordan          & 8,082                   & 351                        & 4.34\%                  \\
% Egypt           & 7,142                   & 207                        & 2.90\%                  \\
% Saudi Arabia    & 4,961                   & 17                         & 0.35\%                  \\
% Palestine       & 2,965                   & 9                          & 0.30\%                  \\ \bottomrule
% \end{tabular}
% \end{table}

% \begin{table*}[h]
% \caption{Primary micro-dialectal intersections by region, reflecting the most fluid linguistic boundaries.}
% \label{tab:dialect_intersections}
% \centering
% \begin{tabular}{@{}lllr@{}}
% \toprule
% \textbf{Region} & \textbf{Dialect A} & \textbf{Dialect B} & \textbf{Overlap Count} \\ \midrule
% \textbf{Jordan}    & Falahi             & Badawi             & 177                    \\
%                    & Falahi             & Madani             & 171                    \\
%                    & Badawi             & Madani             & 23                     \\ \cmidrule(l){2-4} 
% \textbf{Egypt}     & Cairene            & Alexandrian        & 129                    \\
%                    & Cairene            & Port Saidi         & 67                     \\
%                    & Alexandrian        & Port Saidi         & 10                     \\ \cmidrule(l){2-4} 
% \textbf{Saudi}     & Najdi              & Hijazi             & 14                     \\
% \textbf{Palestine} & Madani             & Badawi             & 6                      \\ \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[t!]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.12}

\begin{tabularx}{\textwidth}{@{}
p{1.35cm}
>{\raggedleft\arraybackslash}p{5.15cm}
>{\raggedright\arraybackslash}X
p{2.05cm}
@{}}
\toprule
\textbf{Region} & \textbf{Arabic} & \textbf{English} & \textbf{Multi-label} \\
\midrule

Jordan 
& \setcode{utf8}\<يلا بخاطرك>
& Alright, with your permission 
& Badawi, Falahi \\

Jordan 
& \setcode{utf8}\<اه والله مزبوط>
& Yes by God, it is right 
& Falahi, Madani \\

Egypt 
& \setcode{utf8}\<استنى يابا>
& Wait, father 
& Alex., Port Saidi \\

Egypt 
& \setcode{utf8}\<فلوس باباكي متلزمناش>
& Your father's money does not concern us 
& Alex., Cairene \\

Saudi 
& \setcode{utf8}\<تماما ينطبق نفس الشي على الرجال>
& Exactly the same applies to men 
& Hijazi, Najdi \\

Palestine 
& \setcode{utf8}\<قديش يعني؟ قد البحر. عاد ليش خايف؟>
& How much? As big as the sea. Why are you afraid? 
& Badawi, Madani \\

\blue{Lebanon} 
& \blue{\setcode{utf8}\<بتزين السفرة بهالاشيا>}
& \blue{It decorates the table with these things} 
& \blue{Chamali, Jnoubi} \\

\blue{Mauritania} 
& \blue{\setcode{utf8}\<شوف انا اولدت ف ولاية انشيري >}
& \blue{Look, I was born in Inchiri state} 
& \blue{South., North.} \\

\bottomrule
\end{tabularx}
\caption{Representative multi-label segments in the MicroDA corpus illustrating dialectal convergence.}
\label{tab:multi_label_examples}
\end{table*}

% \begin{table*}[h!]
% \caption{Representative multi-label segments in the MicroDA corpus illustrating dialectal convergence.}
% \label{tab:multi_label_examples}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}llll@{}}
% \toprule
% \textbf{Region} & \textbf{Transcription (Arabic)} & \textbf{Transcription (English)} & \textbf{Multi-Label } \\ \midrule
% Jordan & \setcode{utf8}\hfill \< يلا بخاطرك > & ``Alright, with your permission'' & Badawi, Falahi \\
% Jordan & \setcode{utf8}\hfill \< اه والله مزبوط > & ``Yes by God, it's right'' & Falahi, Madani \\
% Egypt & \setcode{utf8}\hfill \< استنى يابا > & ``Wait, father'' & Alex., Port Saidi \\
% Egypt & \setcode{utf8}\hfill \< فلوس باباكي متلزمناش > & ``Your father's money doesn't concern us'' & Alexandrian, Cairene \\
% Saudi & \setcode{utf8}\hfill \< تماما ينطبق نفس الشي على الرجال > & ``Exactly the same applies to men'' & Hijazi, Najdi \\
% Palestine & \setcode{utf8}\hfill \< قديش يعني ؟ قد البحر. عاد ليش خايف؟ > & ``How much? As big as the sea. Why are you afraid?'' & Badawi, Madani \\
% \blue{Lebanon} & \blue{\<بتزين السفرة بهالاشيا>} & \blue{``It decorates the table with these things''} & \blue{Chamali, Jnoubi} \\
% % Arabic: شوف انا اولدت ف ولاية انشيري انا واحد من اهل انشيري
% \blue{Mauritania} & \blue{\<شوف انا اولدت ف ولاية انشيري انا واحد من اهل انشيري>} & \blue{``Look, I was born in Inchiri state; I am one of the people of Inchiri''} & \blue{Southern, Northern} \\ \bottomrule
% \end{tabular}
% }
% \end{table*}



% I need to write the intersection between countries and between micr-dialects as jaccard idnex



% \subsection{Emotion distribution}


% The stacked distribution in Figure~\ref{fig:emotion_stacked} indicates that \emph{Neutral} dominates across all countries, ranging from 1{,}078 clips in Palestine to 2{,}995 in Jordan. \emph{Anger} is the most prevalent non-neutral emotion and peaks in Jordan (1{,}495 clips), followed by Egypt (1{,}319), with substantially fewer anger clips in  Saudi Arabia (802) and Palestine (503). For \emph{Sadness} and \emph{Happiness}, Egypt has the largest counts (865 and 853, respectively), while \emph{Surprise} is notably high in Saudi Arabia (805) relative to the other countries (691 in Egypt, 448 in Jordan, 248 in Palestine). \emph{Contempt} shows a strong country skew, being most common in Jordan (889) and relatively infrequent in Saudi Arabia (176). Finally, \emph{Fear} remains a low-resource category everywhere (114--377 clips), and \emph{Disgust} is extremely rare (1--26 clips), which makes macro-averaged reporting essential for SER and explains why accuracy alone can be misleading. This imbalance also provides context for the SER benchmarking results in Section~\ref{exp:ser}, where macro-averaged metrics better reflect performance on minority emotions.

% \noindent\textbf{Emotion co-occurrence and ambiguity.} Figure~\ref{fig:emotion_cooccur} makes the multi-emotion nature of many clips explicit: the strongest co-occurrences are between \emph{anger} and \emph{contempt}, and between \emph{sadness} and \emph{neutral}, with additional overlap between \emph{Happiness} and \emph{surprise}. These co-occurrence trends support annotator feedback that utterances are often not well-captured by a single categorical label, and help explain the modest zero-shot SER performance reported in Section~\ref{exp:ser}: when the underlying signal is multi-faceted, single-label evaluation penalizes plausible secondary emotions and increases confusions among adjacent classes (e.g., \emph{sad} vs.\ \emph{neutral}, or \emph{anger} vs.\ \emph{contempt}). In turn, these observations motivate multi-label emotion tags or soft targets that can reflect co-occurring affect and annotator disagreement.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/vertical_distribution_with_counts.pdf}
%     \caption{Stacked distribution of primary emotion labels by country.}
%     \label{fig:emotion_stacked}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/emotion_cooccurrence.pdf}
%     \caption{Emotion co-occurrence patterns across the corpus.}
%     \label{fig:emotion_cooccur}
% \end{figure}



==> Sections/egyptian_dialect.tex <==
\subsection{Egyptian Micro Dialects}
Egyptian dialects are characterized by substantial regional diversity, reflecting geography as well as social, cultural, and historical factors (including internal and external migrations). Pronunciation, lexicon, rhythm, and styles of expression vary across regions. Modern media (cinema and television) have contributed to the spread of a widely understood variety, but it has not erased local distinctions \cite{fashwan2025computational}.  Within Egypt, fine-grained (“micro”) dialect work is facilitated by the fact that the country’s dialect map is described as “relatively well established” due to the \textit{Atlas of Egyptian Rural Arabic} \cite{woidich1996rural} and related work, while earlier linguistic descriptions disproportionately focused on Cairo Arabic and provided comparatively scarcer coverage of regional varieties. Accordingly, microdialectal analysis in Egypt is best framed as (i) adopting the atlas-based geographic skeleton and (ii) grounding micro-variation in diagnostic isoglosses at multiple linguistic levels. 

Following the atlas-based perspective, Egyptian Arabic can be organized by first distinguishing the dialects of the “true Bedouins,” described as groups who arrived relatively recently and live on Egypt’s margins (e.g., Sinai and the Western/Eastern deserts) and are not fully sedentarized \cite{miller2005between}. The atlas then divides the “rural dialects” (sedentary rural population) into three main geographic areas—\textbf{Nile Delta}, \textbf{Nile Valley}, and \textbf{Western Oases}—each with subgroups. In the \textbf{Nile Delta}, the subgroups include \textbf{Western Dialects}, \textbf{North-Eastern Dialects}, \textbf{Central Dialects}, and \textbf{Eastern Dialects}. In the \textbf{Nile Valley}, the atlas distinguishes \textbf{Middle Egypt} dialects (\textbf{NME 1–2, SME}) and \textbf{Upper Egypt} dialects (\textbf{UE 1–4}). \textbf{Western Oases} dialects include four oasis varieties: \textbf{al-Bahariyya, al-Farafra, ad-Dakhla, al-Kharga}. 

Across these regions, reported diagnostic differences include phonological and morphological isoglosses. A widely used macro-isogloss pair is: Cairo / central Delta: /j/ $\rightarrow$ /g/ and /q/ $\rightarrow$ /ʔ/ (e.g., \textit{gamal} ‘camel’, \textit{ʔalb} ‘heart’); versus Sinai Bedouin: /j/ $\rightarrow$ /ʤ/ (or /ʒ/) and /q/ $\rightarrow$ /g/ (e.g., \textit{ʤamal}, \textit{galb}). Another diagnostic concerns the interdentals (θ, ð): Sinai Bedouin is described as retaining interdentals (e.g., \textit{θala:θa} ‘three’, \textit{ðe:l} ‘tail’), whereas Central Delta merges them to /t/ and /d/ (e.g., \textit{tala:ta}, \textit{de:l}). Gender distinctions in plural verbal agreement are reported as retained in some areas but lost/neutralized in others (e.g., Sinai retains masc./fem. plural contrast, whereas central Delta patterns are described as neutralizing it). Morphologically, a diagnostic reported for Qena and farther south, and also in Bahariyya and Farafra, is the “Western imperfect paradigm.” The atlas also points to internal microvariation within Upper Egypt (e.g., UE1 vs.\ UE2). 

In our dataset construction from YouTube speech, we operationalize a complementary, data-driven grouping that aligns with common high-level regional labels while preserving microdialectal coverage in our sampling. Concretely, Egyptian dialects are often classified into three types: \textbf{Cairene} (Cairo), \textbf{coastal dialects} \RL{اللهجات الساحلية} (e.g., Alexandria, Port Said, Ismailia, Sharkia), and \textbf{Saidi} \RL{صعيدى} (Upper Egyptian). Each category exhibits internal variation shaped by city-village differences and regional histories.
\subsubsection{Cairene dialect.}
The Cairo dialect is widely used and prominent, corresponding to Cairo's political, cultural, and media importance; cinema and television have helped popularize and increase comprehension of this dialect \cite{abdel1979comprehensive, el1987egyptian}. It is described as flexible and easy to understand, with a strong ability to absorb new vocabulary from local dialects and other languages, making it a common variety for communication among speakers from different regions.
\subsubsection{Saidi dialect.}
Saidi Egyptian refers to dialects spoken in southern Egypt, particularly in Beni Suef and extending through Minya, Asyut, Sohag, Qena, to Aswan. A key characteristic is the realization of /\RL{ق}/, which is variable in Minya but is described as consistently realized as \RL{ج} in more southern variants \cite{woidich1996rural}. Moving southward, vowel lengthening increases, the pronunciation of emphatic consonants strengthens, and speech patterns become slower and more stable \cite{eida2025beyond}. Despite differences, these dialects share a common phonological framework and are described as showing internally structured regional variation rather than sharply bounded linguistic divisions: from Minya to Aswan, systematic phonological variation forms a geographic continuum.
\subsubsection{Coastal dialects.}
Coastal dialects include those spoken in seashore cities such as Alexandria, Port Said, Damietta, and Marsa Matrouh. They are characterized by historical and cultural influences associated with coastal cities’ openness to trade and contact. The \textbf{Alexandrian dialect} is described as differing from Cairene in rhythm and pronunciation and using local vocabulary related to sea life and trade; it is characterized by a fast rhythm and a relatively sharp tone with clear pronunciation (e.g., a tendency for \RL{ش} and \RL{س} to be pronounced clearly without softening). The \textbf{Port Said dialect} is described as softer in tone with a slightly slower rhythm, including slight elongation in some parts (especially in informal contexts), the use of specific local idioms, and effects from internal migrations reflecting the city’s commercial character and history as an important port.



==> Sections/jordan_dialect.tex <==
\subsection{Jordanian Micro-dialects}
Jordanian Arabic forms a continuum of mutually intelligible dialects across the Kingdom of Jordan, with an emerging common variety alongside significant regional and social sub-varieties that differ in phonological and morphological features \cite{Palva1984,AlWerEtAl2015}. Traditional accounts divide Jordan’s vernaculars into \emph{sedentary} vs.\ \emph{Bedouin} types \cite{Palva1984}: sedentary varieties further split into rural \textit{Falahi} (\<فلاحي>) and urban \textit{Madani} (\<مدني>) dialects, while \textit{Badawi} (\<بدوي>) dialects are associated with nomadic or semi-nomadic tribal origins. In recent decades, strong dialect contact in urban centers,especially Amman, has also produced a mixed koiné that functions as a prestige urban variety \cite{AlWer2007}; below, we overview the three primary micro-dialect groups: Madani, Falahi, and Badawi.

% Jordanian Arabic comprises a continuum of mutually intelligible dialects spoken across the Kingdom of Jordan. Despite an emerging common dialect understood by most Jordanians, there are significant regional and social sub-varieties with distinct phonological and morphological features \cite{Palva1984,AlWerEtAl2015}. Traditionally, scholars divide Jordan's vernaculars into \emph{sedentary} vs. \emph{Bedouin} types, reflecting the historical dichotomy between long-settled communities and nomadic tribes \cite{Palva1984}. The sedentary varieties can be further split into rural \textit{Falahi} (\<فلاحي>, ``peasant'' or rural farmer) dialects and urban \textit{Madani} (\<مدني>, “city dweller”) dialects. Meanwhile, the \textit{Badawi} (\<بدوي>, Bedouin) dialects are associated with tribes of nomadic or semi-nomadic origin. In recent decades, intense dialect contact in urban centers (especially Amman) has led to the formation of a new mixed koiné variety that is widely used as a prestige urban dialect \cite{AlWer2007}. The sections below provide an overview of the three primary Jordanian micro-dialect groups: Madani (Urban), Falahi (Rural), and Badawi (Bedouin).

% \subsubsection{Madani – Urban Koiné Dialect}
% The urban dialect of Amman, the capital and largest city, is often considered a new \emph{koiné} that has emerged from dialect mixing \cite{AlWer2007,AlWer2002b}. Amman was a small town in the early 20th century, but its designation as the capital brought massive migration from various regions: northern Jordan (e.g. Salt and Irbid), southern Jordan (Karak, Ma'an), Bedouin communities, and large waves of Palestinian refugees after 1948 and 1967 \cite{AlWer2007}. As a result, the Ammani dialect is a hybrid combining features from these different dialect sources \cite{AlWer2007,Palva2008}. Notably, the northern Jordan (Horani) input has been very influential in the formation of Amman's speech \cite{AlWer2007}. Over the span of a few decades, the initially mixed dialectal inputs in Amman converged into a stable local variety by the third generation of native Ammani speakers \cite{AlWer2007}. 

% The modern urban Jordanian koiné (exemplified by Ammani speech) is characterized by the reduction or leveling of some marked rural or Bedouin features. For example, traditional northern Jordanian and rural dialects affricate the phoneme /k/ to [\textipa{\t{tS}}] (IPA [\textipa{\t{tS}}], similar to an English “ch”) in front of front vowels (e.g. /keef/ “how” pronounced [\textipa{\t{tS}}i:f]) \cite{Herin2010,HerinAlWer2013,AlHawamdeh2015}. This feature was indeed brought to Amman by early migrants from villages such as Salt, but within the capital it rapidly receded: first-generation Ammanis already shifted /k/ to [k] in all contexts \cite{AlWer2007}. In Amman, affrication became stigmatized as a rural marker, but it is important to note that it continues to be used in other Jordanian cities such as Irbid and Ramtha, especially in semi-urban and rural-urban transitional speech communities \cite{HerinAlWer2013}. 


% Another example of leveling is the second-person plural system. In traditional sedentary Jordanian (Falā\d{h}ī) varieties, speakers distinguish \emph{masculine} /-ku/ vs.\ \emph{feminine} /-ken/, for example [la\textipa{Q}indku] “to your (pl.m) place” vs. [la\textipa{Q}indken] “to your (pl.f) place.” In the north, the /k/ in these endings may undergo affrication before front vowels, producing forms like [la\textipa{Q}ind\textipa{\t{tS}}en] \cite{HerinAlWer2013,herin2014dialect,Palva2008}. In Amman, however, the new urban koiné shows functional neutralization to a single plural form /-kum/, e.g., [la\textipa{Q}indkum], used for both genders in most contexts \cite{AlWer2007}.


% Phonologically, the urban dialects in Jordan share many traits with other Levantine city dialects. One salient feature is the reflex of the letter \textit{qāf} (\<ق>). Urban Jordanian speakers show variation between a glottal stop [\textipa{P}] and [g] for /q/. Studies show that [\textipa{P}] is favored by women, while men more often use [g], and both variants are socially meaningful in Amman speech \cite{AlWerHerin2011,AbdelJawad1986}. The glottal [\textipa{P}] is often heard as indexing urban or Palestinian-oriented identity, whereas [g] indexes a more “tribal” or East Bank identity. Rather than a categorical replacement, Amman thus exhibits stable sociolinguistic variation in (q). 

% Overall, the Madani koiné dialect of Amman has become the prestige urban variety of the capital and a significant source of linguistic influence. However, Falā\d{h}ī and Badawi dialects remain widespread and locally dominant in other towns and regions, and media usage varies by genre (MSA in news, colloquial in entertainment). The Ammani koine therefore serves as a prestigious urban reference point, but coexists with strong Falā\d{h}ī and Badawi varieties in Jordan’s broader dialectal landscape.


\subsubsection{Madani – Urban Koiné Dialect}
The urban dialect of Amman, the capital and largest city, is often described as a new \emph{koiné} that emerged from dialect mixing \cite{AlWer2007,AlWer2002b}. Amman was a small town in the early 20th century, but its designation as the capital brought major migration from northern Jordan (e.g., Salt and Irbid), southern Jordan (Karak, Ma'an), Bedouin communities, and waves of Palestinian refugees after 1948 and 1967 \cite{AlWer2007}. As a result, Ammani speech formed as a hybrid combining features from these sources, with particularly strong influence from northern Jordan (Horani) input \cite{AlWer2007,Palva2008}. Over a few decades, these initially mixed inputs converged into a stable local variety by the third generation of native Ammani speakers \cite{AlWer2007}.

The modern urban Jordanian koiné (exemplified by Ammani speech) is characterized by reduction or leveling of some marked rural or Bedouin features. For example, northern Jordanian and rural dialects may affricate /k/ to [\textipa{\t{tS}}] before front vowels (e.g., /keef/ “how” $\rightarrow$ [\textipa{\t{tS}}i:f]) \cite{Herin2010,HerinAlWer2013,AlHawamdeh2015}. Although this feature was brought to Amman by early migrants (e.g., from Salt), it rapidly receded in the capital: first-generation Ammanis already shifted to [k] in all contexts \cite{AlWer2007}. In Amman, affrication became stigmatized as a rural marker, though it continues in cities such as Irbid and Ramtha, especially in semi-urban and rural--urban transitional communities \cite{HerinAlWer2013}.

Another case of leveling concerns the second-person plural system. Traditional sedentary Jordanian (Falā\d{h}ī) varieties distinguish masculine /-ku/ vs.\ feminine /-ken/ (e.g., [la\textipa{Q}indku] vs.\ [la\textipa{Q}indken]), and in the north /k/ may affricate, yielding forms such as [la\textipa{Q}ind\textipa{\t{tS}}en] \cite{HerinAlWer2013,herin2014dialect,Palva2008}. In Amman, the urban koiné shows functional neutralization to a single plural form /-kum/ (e.g., [la\textipa{Q}indkum]) for both genders in most contexts \cite{AlWer2007}.

Phonologically, urban Jordanian shares traits with other Levantine city dialects, including variation in the reflex of \textit{qāf} (\<ق>) between [\textipa{P}] and [g]. Studies report that [\textipa{P}] is favored by women while men more often use [g], and both variants are socially meaningful in Amman \cite{AlWerHerin2011,AbdelJawad1986}: [\textipa{P}] is associated with an urban or Palestinian-oriented identity, while [g] indexes a more “tribal” or East Bank identity, yielding stable sociolinguistic variation in (q).

Overall, the Madani koiné of Amman has become the prestigious urban variety of the capital and a key source of linguistic influence. At the same time, Falā\d{h}ī and Badawi dialects remain widespread and locally dominant elsewhere, and media usage varies by genre (MSA in news, colloquial in entertainment).

\subsubsection{Falahi – Sedentary Rural Dialects}
The term \textit{Falā\d{h}ī} (“peasant” or rural) refers to the sedentary dialects spoken in Jordan’s villages and smaller towns by non-nomadic communities. These rural dialects are part of the broader Southern Levantine Arabic continuum and share many features with Palestinian rural speech. In northern and central Jordan (historically \textit{\d{H}awrān}, from Amman up to southern Syria), the local rural vernacular is often called the Horani dialect (\textit{\d{h}ōranī} \<حوراني>) \cite{Palva1984}. Horani varieties are characterized by classic Levantine rural features, including /q/ realized as [g] (e.g., \textit{qalb} $\rightarrow$ \textit{galb}) and conditional palatalization (affrication) of /k/ to [t\textipa{S}] before front vowels (e.g., \textit{kīf} $\rightarrow$ \textit{chīf}) \cite{Herin2010,HerinAlWer2013,AlHawamdeh2015}. These features are widespread in northwest Jordan (Irbid, Ajloun, Balqa) and are well documented, though they are often stigmatized, and younger rural speakers frequently adopt urbanized variants in casual speech \cite{AlWer2007}.

Beyond phonetics, Falahi dialects preserve older grammatical distinctions, including gender-specific forms in plural addresses and verb conjugations \cite{AlWer2007}, and they use the proclitic \textit{b-} to mark present-tense verbs (e.g., \textit{b-niktub} “we are writing”), unlike some Bedouin dialects that lack \textit{b-} \cite{AlWerHerin2011}. Lexically, rural Jordanian Arabic overlaps substantially with neighboring Palestinian dialects, alongside localized vocabulary tied to agriculture and village life. Sedentary dialects are not monolithic: there is notable sub-regional variation (e.g., far north vs.\ the Karak plateau), including regional realizations of the feminine ending “-a” (tā\textsuperscript{'} marbū\d{t}a), raised to [e] in southern rural Jordan (\textit{maktabe}) and often realized as a more central [æ] in northern dialects (\textit{maktabeh}), in contrast to Bedouin [a] \cite{Palva2008}. Nevertheless, Falahi varieties remain mutually intelligible within the broader sedentary Levantine type, and many rural speakers are bidialectal, using the local dialect at home but shifting towards urban speech in formal settings or when interacting with outsiders.



\subsubsection{Badawi – Bedouin Dialects}
The Bedouin dialects of Jordan are associated with Bedouin tribes, traditionally pastoral nomads of the eastern deserts and southern steppe. Linguistically, they fall under Arabian Bedouin Arabic and are often classified as “Northwest Arabian” Arabic \cite{Palva2008}. In Palva’s classification, the Bedouin-type dialects spoken in Jordan (and neighboring desert regions of Syria and Arabia) form an eastern subgroup of Northwest Arabian dialects \cite{Palva2008,HerinEtAl2022} and show strong affinities with the dialects of the Negev, Sinai, and the Najd rather than with sedentary Levantine city and village dialects \cite{Palva2008,HerinEtAl2022}. Within Jordan, Bedouin varieties further differ along tribal lines and historical origins: southern Jordan dialects (e.g., \d{H}uway\d{t}āt, Banī 'A\d{t}iyyah, the Bdul of Petra, and the 'Nmāt) share features with Sinai and Negev Bedouin \cite{Palva2008}, while major tribes in central and northern Jordan (e.g., Banī \d{S}axr, Banī \d{H}asan, Sir\d{h}ān) speak North Arabian (Najdi)–type dialects associated with the 'Anaza and Shammār confederations \cite{HerinEtAl2022}. Some north-eastern Bedouin communities (e.g., Sir\d{h}ān of the \d{H}amād) speak \textit{šāwī} Arabic, similar to Syrian–Iraqi Bedouin dialects and often distinguished by plural verb forms ending in -\textit{ūn} (e.g., \textit{yīgūlūn} “they say”) \cite{HerinEtAl2022}.

Despite local differences, Jordanian Bedouin dialects share defining features. Phonetically, /q/ is typically realized as [g] (e.g., \textit{gabīl} for \textit{qabīl} “before”), and /k/ generally remains [k] (with /k/-palatalization described as rare and largely limited to certain words or older speakers). They also tend to preserve classical vowel features reduced in sedentary speech; for instance, /aw/ and /ay/ may be retained as diphthongs or only partially monophthongized, whereas urban Jordanian often realizes them as [\textipa{o:}] and [\textipa{e:}] \cite{Palva2008}. Grammatically, Bedouin varieties often lack (or optionally use) the habitual \textit{b-} prefix on present tense verbs, using forms such as \textit{aktub} or an auxiliary (e.g., \textit{gā\textipa{P}id aktub}, “I am writing”) \cite{AlWerHerin2011}, and they preserve lexical items and idioms tied to desert life. Although many Bedouin groups have become settled and dialect contact has led to gradual convergence in some communities \cite{HerinEtAl2022}, core Bedouin features remain salient identity markers (e.g., [g] vs.\ [\textipa{P}] for /q/), and many speakers are bidialectal, using Badawi at home and shifting to the urban koine in mixed settings.




% \subsubsection{Falahi – Sedentary Rural Dialects}
% The term \textit{Falā\d{h}ī} (“peasant” or rural) refers to the sedentary dialects spoken in Jordan’s villages and smaller towns by non-nomadic communities. These rural dialects form part of the broader Southern Levantine Arabic continuum, sharing many features with Palestinian rural speech. In northern and central Jordan (the region historically known as \textit{\d{H}awrān}, spanning from Amman up to southern Syria), the local rural vernacular is often called the Horani dialect (\textit{\d{h}ōranī} \<حوراني>) \cite{Palva1984}. Horani (northern Jordanian) varieties are characterized by several classic Levantine rural features. One hallmark is the realization of the classical /q/ as a voiced velar [g]. For example, \textit{qalb} “heart” is pronounced \textit{galb} in rural Jordanian. Another is the conditional palatalization (affrication) of /k/ to [t\textipa{S}] before front vowels, as in \textit{kīf} “how” $\to$ \textit{chīf} \cite{Herin2010,HerinAlWer2013,AlHawamdeh2015}. These features are widespread across villages in northwest Jordan (Irbid, Ajloun, Balqa) and have been documented extensively in dialectological studies \cite{Herin2010,HerinAlWer2013,AlHawamdeh2015}. However, they are often stigmatized, and younger rural speakers frequently adopt urbanized variants in casual speech \cite{AlWer2007}. 

% In addition to phonetic traits, Falahi dialects preserve some older Arabic grammatical distinctions. As noted above, traditional rural speech maintains gender-specific forms in plural addresses and verb conjugations (using feminine plural endings when speaking to or about groups of women) \cite{AlWer2007}. Rural dialects also universally use the proclitic \textit{b-} to mark present-tense verbs (e.g. \textit{b-niktub} “we are writing”), a feature shared with urban Levantine dialects but in contrast to some Bedouin dialects which lack the \textit{b-} prefix \cite{AlWerHerin2011}. Lexically, rural Jordanian Arabic has much in common with neighboring Palestinian dialects, though one can find localized vocabulary related to agriculture and village life. 

% It should be noted that the sedentary dialects in Jordan are not monolithic; there is considerable sub-regional variation. The rural speech of the far north (Irbid and surroundings) versus the south (e.g. the Karak plateau) differs in accent and certain vowel patterns. For example, the pronunciation of the feminine ending “-a” (the tā\textsuperscript{'} marbū\d{t}a) varies regionally: in southern rural Jordan it is raised to [e] (e.g. \textit{maktaba} “library” becomes \textit{maktabe}), whereas northern dialects often realize it as a more central [æ] (\textit{maktabeh}), in contrast to the Bedouin pronunciation [a] \cite{Palva2008}. Such differences distinguish micro-dialects between localities. Nevertheless, all Falahi varieties in Jordan are mutually intelligible and belong to the broader sedentary Levantine type. Many speakers from rural areas are bidialectal, using their local dialect at home but switching toward urban speech in formal settings or when interacting with outsiders.

% \subsubsection{Badawi – Bedouin Dialects}
% The Bedouin dialects of Jordan are those associated with the Bedouin tribes, traditionally pastoral nomads of the eastern deserts and southern steppe regions. Linguistically, these dialects fall under the umbrella of Arabian Bedouin Arabic and are often classified as part of “Northwest Arabian” Arabic \cite{Palva2008}. According to Palva's classification, the Bedouin-type dialects spoken in Jordan (and neighboring desert regions of Syria and Arabia) constitute an eastern subgroup of Northwest Arabian dialects \cite{Palva2008,HerinEtAl2022}. They show strong affinities with the dialects of the Negev, Sinai, and the Najd, rather than with the sedentary Levantine dialects of the cities and villages \cite{Palva2008,HerinEtAl2022}. Within Jordan, Bedouin varieties can be further divided along tribal lines and historical origins. For instance, the dialects of southern Jordan (spoken by clans such as the \d{H}uway\d{t}āt, Banī 'A\d{t}iyyah, the Bdul of Petra, and the 'Nmāt) share features with those of the Sinai and Negev Bedouin \cite{Palva2008}. In central and northern Jordan, major tribes like the Banī \d{S}axr, Banī \d{H}asan, and Sir\d{h}ān speak dialects of the North Arabian (Najdi) type associated with the 'Anaza and Shammār confederations \cite{HerinEtAl2022}. Additionally, some Bedouin communities in the north-east (e.g. the Sir\d{h}ān of the \d{H}amād desert) speak \textit{šāwī} Arabic, which has similarities to Syrian–Iraqi Bedouin dialects (often distinguished by plural verb forms ending in -\textit{ūn}, as in \textit{yīgūlūn} “they say”) \cite{HerinEtAl2022}. 

% Despite local sub-differences, Jordanian Bedouin dialects share a number of defining features. Phonetically, they typically realize /q/ as [g], a trait common to most Bedouin and rural dialects (e.g. \textit{gabīl} for \textit{qabīl} “before”). The pronunciation of /k/ remains [k] in Bedouin speech, unlike the [t\textipa{S}] affrication of sedentary dialects; historical traces of /k/-palatalization are rare and mostly confined to certain words or older speakers. Bedouin dialects also tend to preserve classical Arabic vowel features that have been reduced in sedentary speech. For example, the old diphthongs /aw/ and /ay/ may be retained as diphthongs or only partially monophthongized, whereas urban Jordanian dialects typically realize them as [\textipa{o:}] and [\textipa{e:}] \cite{Palva2008}. In terms of grammar, Bedouin varieties are often more conservative or employ different particles. A well-known difference is the absence (or optional use) of the habitual \textit{b-} prefix on present tense verbs. Instead of saying \textit{baktub} “I write” as in Falahi or Madani speech, a Bedouin speaker might say \textit{aktub} or use an auxiliary (e.g. \textit{gā\textipa{P}id aktub}, “I am writing”) \cite{AlWerHerin2011}. Bedouin dialects also preserve certain lexical items and idioms related to desert life that differ from those in sedentary vocabulary. 

% Many Bedouin groups in Jordan have become settled over the past century, bringing their dialects into close contact with rural and urban varieties. Consequently, researchers have observed a gradual convergence in some communities \cite{HerinEtAl2022}. Nevertheless, core Bedouin features remain robust markers of identity. In Jordan, speakers can often readily tell a Bedouin-accented person from an urban one by the use of [g] vs [\textipa{P}] for /q/, along with certain intonation patterns and tribal idioms. The Badawi dialects continue to be proudly used within Bedouin communities and in cultural settings (such as oral poetry and traditional songs), while many Bedouin speakers are bidialectal—using their dialect at home but switching to the urban koine in mixed settings or when addressing non-Bedouin Jordanians.



% \subsection{Overview of Jordanian Micro-dialects}

% Jordanian Arabic is not a single homogeneous dialect but a continuum of \textbf{micro-dialects} shaped by historical settlement patterns and social identity. Broadly, scholars distinguish three primary varieties in Jordan: \textbf{Madani (Urban)}, \textbf{Falahi (Sedentary Rural)}, and \textbf{Badawi (Bedouin)} dialects. This tripartite division corresponds to the country’s social history: urban centers that emerged in the 20th century, long-established farming villages, and nomadic or tribal communities \citep{AbdelJawad1986}. Each variety has distinct linguistic features and sociolinguistic significance, though contact and migration have increasingly blurred strict boundaries \citep{AlWer2007,AlWerHerin2011}.

% \subsubsection{Madani – Urban Koine}

% The term \textit{Madani} (\<مدني>, ``urban'') refers to the dialects of the cities. In Jordan, urban dialects are relatively new, as major urbanization only occurred in the 20th century. Amman – a small town with no indigenous Arabic dialect at the start of the 1900s – became the capital in 1921 and rapidly grew into a melting pot of speakers from different regions \citep{AlWer2007}. The result was the formation of a new \textbf{urban koine} in Amman (and other towns like Zarqa and Irbid) that merges features from various dialect sources \citep{AbdelJawad1986}. This \textbf{Modern Jordanian Urban} dialect (often just called ``Ammani'') is now the most common spoken variety among Jordanians in daily life \citep{AlWer2007}.

% Historically, the Ammani koine emerged from contact between local Transjordanian dialects and the dialects of waves of immigrants. In the early to mid-20th century, many Jordanians from the northern \textbf{Horān} region (northwest Jordan/southern Syria) and other parts of the country moved to Amman, followed by large influxes of Palestinian refugees after 1948 and 1967 \citep{AlKhatib1988}. The northern Horani dialect in particular had a strong influence on the nascent urban speech \citep{AlWer2007}. Horani (spoken in areas from Amman up to Irbid and across the Horan plateau) is a sedentary rural dialect characterized by features like pronunciation of \textit{qāf} /q/ as [g] and palatalization of /k/ to [t\textipa{S}] before front vowels \citep{HerinAlWer2013}.

% Urban Palestinian dialects contributed features such as the realization of /q/ as [\textipa{P}] and certain vowel shifts \citep{AlWerHerin2011}. The coexistence of speakers from East Bank (Transjordanian) origin – who tended to use [g] for /q/ – and those from Palestinian origin – often using [\textipa{P}] for /q/ – led to a \textbf{stable variation} in the new city dialect. Studies by Al-Wer and Herin document how these variants became \textbf{socially stratified}: [g] is associated with local Jordanian identity and [\textipa{P}] with Palestinian identity \citep{AlWerHerin2011}. By the third generation of Ammanis, a focused dialectal norm had emerged \citep{AlWer2007}.

% Phonologically, aside from the variable (q) realization, urban Jordanian tends to lack the heavy affrication of /k/ that Horani village dialects have; younger speakers in cities increasingly pronounce /k/ as [k] rather than [t\textipa{S}], a change observed in towns like Salt \citep{HerinAlWer2013}. Urban dialects also typically drop interdental fricatives (\textipa{T}, ð) in favor of dental stops, aligning with Levantine city dialects. Morphosyntactically, the urban koine shows leveled forms, such as uniform second person plural suffix -ku \citep{AbdelJawad1986}. The prefix \textit{b-} on present tense verbs (e.g. \textit{biktib} ``he writes'') is nearly categorical in urban speech \citep{AlWerHerin2011}.

% Sociolinguistically, the rise of the Madani koine has led to the \textbf{urban dialect becoming the overt prestige variety} in Jordan \citep{AbdelJawad1986}. Speakers from rural or Bedouin backgrounds often accommodate toward urban norms, especially younger generations. However, there is also evidence of \textbf{covert prestige} for non-urban features: some speakers (particularly of Bedouin origin) may pride themselves on using [g] as an index of authentic Jordanian heritage \citep{AlWerEtAl2015}.

% \subsubsection{Falahi – Sedentary Rural Speech}

% The term \textit{Falahi} (\<فلاحي>, ``rural'') refers to the sedentary rural dialects spoken by villagers and agricultural communities. In the Jordanian context, Falahi often specifically evokes rural Palestinian dialects, because many Jordan’s population has roots in Palestinian villages \citep{AlKhatib1988}. Researchers distinguish between local Horani villagers and Palestinian \textit{fellah} speakers \citep{AlKhatib1988}.

% Falahi dialects are marked by the treatment of /q/. In central Palestinian rural speech, /q/ is realized as [k] (``bikul'' dialects), while in northern Jordanian and southern Palestinian villages it is [g] (``bigul'' dialects) \citep{AbdelJawad1986}. Horani dialects are also known for affricating /k/ to [t\textipa{S}] before front vowels \citep{HerinAlWer2013}. However, this affrication is receding under urban influence \citep{HerinAlWer2013}.

% Falahi dialects preserve conservative morphosyntax in some respects, such as the use of \textit{b-} on present tense verbs, and retention of distinct feminine plural forms in more isolated villages \citep{AbdelJawad1986}. Lexically, they include vocabulary tied to agriculture and rural life. Socially, Falahi speech often indexes local identity, though urban speech has higher prestige \citep{AlWerEtAl2015}.

% \subsection{Badawi – Bedouin Dialects}

% Badawi dialects are the traditional dialects of nomadic or formerly nomadic tribes in Jordan, belonging to the Arabian Bedouin Arabic continuum. In Jordan, Bedouin tribes ranged across the eastern steppe and southern deserts. Their speech is distinct from sedentary dialects \citep{AbdelJawad1986}.

% A defining feature of Bedouin dialects is the pronunciation of /q/ as [g]. Bedouin dialects typically lack the prefix \textit{b-} on imperfect verbs (e.g., \textit{yiḥki} vs. urban \textit{biḥki}) \citep{AbdelJawad1986}. They also preserve the interdental fricatives /θ/ and /ð/ \citep{AlWerEtAl2015}. Bedouin speech tends to retain final vowels, such as feminine -a, in contrast to sedentary [-e] or [-eh] variants \citep{HerinAlWer2013}.

% Jordan’s Bedouin dialects can be divided into Southern Bedouin (linked to Hijazi and Negev Arabic) and Northern/Central Bedouin (linked to Najdi and Shawi varieties) \citep{AlWerEtAl2015}. Despite internal diversity, all Bedouin dialects share traits distinguishing them from Madani and Falahi. Sociolinguistically, Bedouin speech has historically been stigmatized as harsh, but it also indexes authenticity and heritage \citep{AlWerEtAl2015}.



% ----------------
% ----------------
% ----------------
% ----------------


% \subsubsection{Madani – Urban Koiné Dialect}
% The urban dialect of Amman -- the capital and largest city -- is often considered a new \emph{koiné} that has emerged from dialect mixing \cite{AlWer2007,AlWer2002b}. Amman was a small town in the early 20th century, but its designation as the capital brought massive migration from various regions: northern Jordan (e.g. Salt and Irbid), southern Jordan (Karak, Ma'an), Bedouin communities, and large waves of Palestinian refugees after 1948 and 1967 \cite{AlWer2007}. As a result, the Ammani dialect is a hybrid combining features from these different dialect sources \cite{AlWer2007,Palva2008}. Notably, the northern Jordan (Horani) input has been very influential in the formation of Amman's speech \cite{AlWer2007}. Over the span of a few decades, the initially mixed dialectal inputs in Amman converged into a stable local variety by the third generation of native Ammani speakers \cite{AlWer2007}. 

% The modern urban Jordanian koiné (exemplified by Ammani speech) is characterized by the loss or leveling of many marked rural or Bedouin features. For example, traditional rural dialects affricate the phoneme /k/ to [t\textipa{S}] (IPA [\textipa{\t{tS}}], similar to an English “ch”) in front of front vowels (e.g. /keef/ “how” pronounced [t\textipa{S}īf]) \cite{Herin2010,HerinAlWer2013,AlHawamdeh2015}. This feature was brought to Amman by early migrants from villages (e.g. the city of Salt), but it quickly disappeared in the urban environment: first-generation Ammanis already “deaffricated” /k/ to [k] in all contexts \cite{AlWer2007}. Affrication of /k/ is stigmatized as a rural feature, and accordingly it is not found in any Jordanian city dialect \cite{AlWer2007}. Another example of leveling is the loss of gender-specific plural forms. In traditional Jordanian Arabic, speakers maintain a distinction between masculine and feminine in second- and third-person plural pronouns and verb agreements (e.g. \textit{\textipa{P}intu} “you (pl.m)” vs. \textit{\textipa{P}intin} “you (pl.f)”) \cite{AlWer2007}. The Ammani koine, like other urban Levantine dialects, has neutralized these to a single form (using \textit{\textipa{P}intu} for “you (pl)” regardless of gender) \cite{AlWer2007,AlWer2003}. 

% Phonologically, the urban dialects in Jordan share many traits with other Levantine city dialects. One salient feature is the reflex of the letter \textit{qāf} (\<ق>). Urban Jordanian speakers typically use a glottal stop [\textipa{P}] for /q/ (as in \textit{\textipa{P}ahwe} for \textit{qahwa} “coffee”), a feature associated with Levantine urban prestige norms and reinforced by the influence of Palestinian dialects. In contrast, rural and Bedouin Jordanians usually pronounce /q/ as [g] (see below). This difference in the realization of /q/ has taken on social significance in Jordan: the glottal [\textipa{P}] is often heard as a marker of urban or Palestinian-affiliated speech, whereas [g] signals a more “tribal” or East Bank identity \cite{AlWerEtAl2015,AlWerHerin2011}. Indeed, certain lexical variants in the Ammani koine can be traced to either Jordanian or Palestinian provenance. For example, some distinctly Palestinian features present in first-generation Ammanis were largely eliminated in subsequent generations \cite{AlWer2002b}. Overall, the Madani koine dialect of Amman has become the dominant spoken variety in media and daily life in Jordan's cities. It serves as a lingua franca among Jordanians of different backgrounds, and younger Jordanians even in smaller towns increasingly adopt Ammani features in informal speech.

==> Sections/palestinian_dialect.tex <==
\subsection{Palestinian Micro-dialects}

Palestinian Arabic forms a continuum of related dialects across Palestine, with regional and social variations shaped by urbanization,village ties, and the dialect contact produced by forced displacement after the 1948 Nakba \cite{Shahin2008,CotterHoresh2015}. Traditional descriptions often divide Palestinian everyday speech into \emph{urban} vs.\ \emph{rural} types through clear phonological features. However, this binary captures only part of the variation, as many speakers combine features from different local and social backgrounds.
To represent this variation, we adopt a three-part classification: urban speech, northern rural speech, and southern rural speech. This classification is not a fixed geographic map; rather, it reflects recurring patterns of linguistic co-occurrence in pronunciation, negation, lexical choice, and grammar \cite{JHRAZ17}.

\paragraph{Madani (Urban)}

From Jerusalem, Nablus, and Hebron in the highlands to Gaza City on the coast, and from Jaffa to the northern urban corridor of Nazareth and Haifa, Palestinian urban dialects represent more than geographical variation; they reflect a linguistic ecology shaped by long-run urbanization, social mobility, and trade networks \cite{Shahin2008}.

Palestinian cities have long functioned as magnets for migration from surrounding villages, as refuges during periods of displacement, where families from different regional backgrounds formed shared patterns of urban speech. This urban voice carries within it the echoes of Nablusi merchant families, Jerusalem religious scholars, Gazan fishing communities, and Jaffan citrus farmers, all woven into a recognizable city sound that now extends across the Palestinian landscape.

The phonological signature of this urban dialect is most audible in its treatment of the historical consonant \<ق> (\textit{q\=af}), which shifts from its Classical uvular articulation to a glottal stop [\textglotstop]; thus \<قلب> \textit{qalb} (heart) becomes \textit{\textglotstop{}alb}, written in Arabic script as \<قلب> but pronounced as \textit{\textglotstop{}alb} \cite{Shahin2008}.

This variable serves as a major marker of Palestinian urban speech. The urban profile is also reflected in the simplified realization of \<ث> (\textit{th\=a'}) and \<ذ> (\textit{dh\=al}) in frequent words, such as \<كثير> \textit{kath\=ir} ``many'' realized as \textit{kt\=ir}, and \<هذا> \textit{h\=adh\=a} ``this'' as \textit{h\=ada}. Together, these features shape the phonological profile of urban Palestinian Arabic \cite{AlWer2003}.

This urban voice does not echo only within city centers. It radiates outward, diffusing through what might be called the semi-urban landscape: the towns climbing the hills around Ramallah, the mixed cities where refugee camps press against municipal boundaries. The result is a landscape of hybrid speech that resists easy classification as purely ``city'' or purely ``village''. Overall, Madani has crystallized as the prestigious urban voice of Palestine's historic city centers, while rural dialects remain locally dominant across rural landscapes.

\paragraph{Northern (Fallahi)}

The rural dialects of northern Palestine constitute a distinct linguistic system, stretching from the Jenin highlands through the villages of Tulkarm, Qalqilya, and Salfit, and extending northward into the Galilean communities around Nazareth and the Triangle region. These varieties have clear pronunciation patterns linked to village identity. The chain shift is seen when the historical \<ق> (\textit{q\=af}) is often pronounced like [k], while \<ك> (\textit{k\=af}) is sometimes pronounced like a ``ch'' sound [\textipa{\t{tS}}], as in \textit{chif} for ``how'' (\<كيف>), compared with the urban \textit{keef}. This coupled shift creates a network of contrasts in which minimal pairs are distinguished not by context alone, but by a systematic redistribution of phonological cues: \textit{qalb} (\<قلب>, heart) surfaces as \textit{kalb}, while \textit{kalb} (\<كلب>, dog) may surface as \textit{chalb}, preserving the contrast through affrication \cite{jarrar-etal-2014-building}.

Negation patterns show a similar structure: the circumfix \textit{ma-...-\v{s}} wraps around verbs with greater consistency, as in \textit{ba'rif-\v{s}} ``I do not know'', while existential negation employs forms such as \textit{ma-f\=i\v{s}(-\v{s})}. In agreement, rural speech maintains distinctions that urban speech has often leveled: feminine plural subjects trigger feminine plural marking on verbs and adjectives, as in \textit{il-ban\=at r\=ahn} ``the girls went'' and \textit{il-ban\=at ta'b\=an\=at} ``the girls are tired'' \cite{JHRAZ17}.

Like its urban counterpart, this rural voice does not remain static within village boundaries. It travels with speakers into cities, mixed towns, and camps. Overall, the northern \textit{Fall\=ah\=i} variety remains locally dominant across the West Bank northern highlands, Galilean hills, and the villages of the Triangle, while urban varieties claim the cities and Modern Standard Arabic holds its domain in formal media.

\paragraph{Southern (Badawi)}

South of Jerusalem, the linguistic landscape changes. In the villages of Arab al-Saw\=ahirah overlooking the Holy City, across Arab al-Ta'\=am\=irah and Ban\={\i} 'Ubayd in the Bethlehem countryside, and onward into the Hebron highlands (Yatta, Dura, al-Dhah\={a}hiriyya, Ban\={\i} Na'\={\i}m), the southern rural voice of Palestine takes on distinct contours. Its reach extends southwest toward Beer al-Saba', where Naqab tribes maintain strong tribal speech patterns, and westward into Gaza, where displaced families have contributed to the speech patterns of camps and coastal cities \cite{Cotter2022}.

The phonological signature of this continuum is marked by the realization of \<ق> (\textit{q\=af}). Unlike northern rural varieties, where /q/ often shifts to /k/, and urban varieties, where it often becomes a glottal stop [\textglotstop], southern rural speech commonly realizes /q/ as [g]; thus \<قلب> \textit{qalb} ``heart'' may surface as \textit{galb} \cite{Shahin2008}. This pattern is accompanied by greater preservation of \<ث> (\textit{th\=a'}) and \<ذ> (\textit{dh\=al}) in frequent words, as in \<كثير> \textit{kath\=ir} ``many'', which may surface as \textit{ka\texttheta\=ir} rather than urban \textit{kt\=ir}, and \<هذا> \textit{h\=adh\=a} ``this'', which may surface as \textit{h\=adha} rather than \textit{h\=ada}. Similar preservation appears in numerals such as \<ثلاثة> \textit{thal\=atha} ``three'', compared with urban forms like \<تلاتة> \cite{AlWer2003}.

Alongside these phonological cues, a set of lexical choices strengthens the overall signature. Speakers may use \<هلحين> \textit{\d{h}al\d{h}\=in} ``now'', contrasting with northern rural \<هسا> \textit{hassa} and urban \<هلأ> \textit{halla\textglotstop{}}. Temporal interrogation may favor \<وقتيش> \textit{wagt\=e\v{s}} ``when'', contrasting with northern \<وينتا> \textit{w\=enta} and urban \<ايمتا> \textit{aymt\=a}. The everyday verb ``look'' can also index region, with southern speech using items such as \<بحِّر> \textit{ba\d{h}\d{h}ir} alongside other Palestine-wide options like \<اطّلع> \textit{i\d{t}\d{t}alla'} and \<شوف> \textit{\v{s}\=uf} \cite{JHRAZ17}. Taken together, these choices form an acoustic signature that many listeners recognize quickly as ``southern rural''.

This southern voice flows beyond village and tribal boundaries in Palestine. Shaped by centuries of contact with neighboring Bedouin dialects from southern Jordan to northern Saudi Arabia, and from Sinai to the Nile Delta. It remains an important marker of rural and tribal identity \cite{Palva2008}.

Taken together, Palestinian micro-dialects are best understood as a continuum rather than as isolated categories. Urban, northern rural, and southern rural varieties, alongside Modern Standard Arabic in formal domains, they shape the broader linguistic landscape of Palestine \cite{jarrar-etal-2014-building}.

==> Sections/saudi_dialect.tex <==
\subsection{Saudi micro-dialects}

 The categorization of Saudi Arabian dialects into different regions is a conventional method used in modern sociolinguistic and phonetic research \cite{ingham1994najdi,Prochazka1988}. The dominant classification in current research encompasses the Najdi, Hijazi, Eastern, Northern, and Southern dialects. Each dialect reflects unique characteristics across the levels of linguistic analysis. The following is a summary of each dialect group.

\subsection{Najdi}
The Najdi dialect is spoken across central Saudi Arabia and can be divided into four main regional varieties \cite{ingham1994najdi}: Central Najdi (spoken in the heart of Najd), Northern Najdi (linked to the Jabal Shammar and ha'il area), Mixed Northern-Central Najdi (common in the Qassim region), and Southern Najdi (extending to southern areas such as Najran).

Northern Najdi is primarily spoken in the ha'il region and surrounding northern areas \cite{ingham1994najdi}. It retains many conservative and Bedouin features, including traditional vocabulary and expressions passed down through generations. The Mixed Northern-Central Najdi dialect, centered in the Qassim region, is characterized by distinctive pronunciation patterns, such as the affrication of certain consonants, and a unique melodic intonation. This variety reflects a blend of both northern and central Najdi, shaped by internal migration and trade \cite{ingham1994najdi}. Central Najdi, dominant in the capital city Riyadh and its surrounding towns, is considered the standard variety of Najdi Arabic. Due to Riyadh’s political and economic prominence, this dialect has become associated with formal communication \cite{ingham1994najdi, Prochazka1988}. Finally, Southern Najdi, spoken along the southern edges of Najd and extending toward Najran, preserves older features that are less common in urban centers and shows some influence from southern Arabian dialects \cite{ingham1994najdi}.

In some Najdi dialects (more dominantly Qassimi dialect), the sound \textipa{/k/} is often 
realized as \textipa{[ts]}; for example, a word pronounced as 
\textipa{/kaD."Da:b/} \<كذاب> in MSA may be realized as 
\textipa{[tsaD."Da:b]} \<تسذاب> in Najdi speech. Similarly, the greeting 
\textipa{/\v{s}.lo:.nak/} \<شلونك> (when addressing a female) may be 
realized as \textipa{[\v{s}.lo:.nats]} \<شلونتس> in some Najdi dialects.

\subsection{Hijazi}

Another major part of Saudi Arabia is the Hijaz region, which is a historically significant region in western Saudi Arabia that stretches along the Red Sea coast and encompasses the major cities of Mecca, Medina, Jeddah, Yanbu, and Taif, as well as the surrounding tribal areas \cite{destinationksa_hejaz}. Linguistically, the region is far from homogenous. The ``Hijazi dialect'' is not a single variety but rather a collection of dialects that can be grouped into two main categories \cite{sambas2016hijazi}: 1) The Urban Hijazi which is spoken in the large cities of Mecca, Medina, Jeddah, Taif, and Yanbu. These cities have long attracted Arabs and Muslims, whether to live in proximity to the holy sanctuaries of Mecca and Medina or for economic and social opportunities, creating a speech variety shaped by both native residents and long-term settlers. This is the dialect that most people typically identify as ``Hijazi Arabic.'' 2) The tribal Hijazi which is Associated with the speech of Bedouin tribes inhabiting the broader Hijaz region. These dialects preserve Bedouin phonological and morphological features and are spoken by tribal groups whether in rural areas or, in some cases, within urban settlements.




In the Hijazi dialect, the sound \textipa{/D/} is 
often realized as \textipa{[z]}; for example, a word pronounced as  
\textipa{/kaD."Da:b/} \<كذاب> is frequently pronounced as 
\textipa{[kaz."za:b]} in Hijazi speech. Another characteristic feature is the substitution of \textipa{/T/} with 
\textipa{[t]}; for example, a word pronounced as \textipa{/Ta.la:.Ta/} 
\<ثلاثة>  may be realized as \textipa{[ta.la:.ta]} 
in Hijazi speech.


\subsection{Eastern}
The Eastern dialect of Saudi Arabia is primarily spoken in the Eastern Province, including key cities and regions such as Dammam, Al-Ahsa (Hofuf), Qatif, and Khobar. The Eastern dialect is very similar to other countries in the Gulf region, such as Bahrain and Qatar \cite{gulfarabicresources}. This can be attributed to the boarder shared between Saudi and Bahrain and Saudi and Qatar. 

Socially, the Eastern dialect is often described as slow in tempo, contrasting with the faster, more clipped rhythm of other dialects such as Najdi or Southern Arabic. Vowel quality in Eastern Arabic is notably distinct. The /\textipa{a}/ sound in medial syllables can be rounded, while in final position it may appear as a more open /\textipa{a:}/, imparting a unique musicality to the dialect. Additionally, the Eastern dialect is known for preserving some conservative phonetic and lexical features that have evolved or disappeared in other Saudi dialects. For instance, certain traditional vocabulary items such as the word ``simat'' (meaning `dining mat'), are still used in the Eastern region but are rarely heard in other parts of Saudi Arabia. Additionally, a word such as \textipa{/kaDDab/} \<كذاب> may be realized as \textipa{[tSaDDab]} \<تشذاب>.



\subsection{Southern}
The Southern dialect of Saudi Arabia is spoken in the southern regions, notably in cities and areas such as Abha, Khamis Mushait, Jazan, Najran. This dialect is closest to the Yemeni dialect \cite{asiri2009}. The southern dialect can be further divided into Asiri (spoken in the highlands near Abha), Tihami (along the Red Sea coastal plain), Najrani (in Najran), and Jizani (in Jazan) \cite{alqahtani2015tihami}. The Southern dialect is often recognized for its fast and clipped rhythm. Phonological studies have shown that southern dialects may retain or develop consonantal and vowel features that are rare in other parts of Saudi Arabia, such as unique realizations of /q/.

The Asiri dialect is mostly spoken in cities such as Abha and Khamis Mushait. It maintains traditional Arabic features, including gender and plural distinctions in verbs and pronouns \cite{asiri2009}. The Tihami dialect is spoken along the Red Sea coastal plain, spanning the lowlands of western Asir and part of Jazan. It is notable for its rapid, clipped rhythm and simplified syllable structure. The Najrani and Jizani dialects have a similar grammar and vocabulary to Yemeni Arabic, a result of longstanding cultural and geographic proximity to Yemen.

In some Southern dialects, the greeting 
\textipa{/kay.fa \textsl{h}a:.lak/} \<كيف حالك> (when addressing a female) 
is often pronounced as \textipa{[kayf \textsl{h}a:.la\v{s}]} \<كيف حالش>. 
This reflects a common shift where the final ``k'' sound changes into a 
``sh'' sound. This feature, known as \textit{kashkasha}, is a well-known 
characteristic of speech of the Southern dialect.




\subsection{Northern}
The Northern dialect of Saudi Arabia is predominantly spoken in the northern regions, including cities and areas such as Tabuk, Arar, Al-Jawf, Rafha, and the surrounding rural communities. Al-Jawf dialect is  influenced by its proximity to Jordan, Syria, and Iraq \cite{north_Dialect}. However, dialects spoken in Arar, Tabuk, and Rafha are very similar to Ha'il dialect.  

Linguistically, the Northern dialect exhibits several salient features. There is often a rising intonation in speech, and certain words or pronunciations may be hard for speakers from other Saudi regions to fully grasp. The Northern dialect is often associated with Bedouin heritage and retains many traditional speech patterns reflective of the nomadic lifestyle prevalent in these regions. 

In some Northern dialects,  the sound \textipa{/k/} is often 
realized as  \textipa{[ts]}; for example, a word pronounced as 
\textipa{/kaD."Da:b/} \<كذاب>  may be realized as 
\textipa{[tsaD."Da:b]} \<تسذاب> in Northern speech, similar to some Najdi dialect. Similarly, the greeting 
\textipa{/\v{s}ax.ba:.rak/} \<شخبارك> (when addressing a female) may be 
realized as \textipa{[\v{s}ax.ba:.rats]} \<شخبارتس>. 


%%%%%%%%%%%%%%%%%%%

% In this section, we provide a general overview of the micro-dialects spoken in Saudi Arabia. In the existing literature, there is some variations in how the dialects of Saudi Arabia are broadly categorized. Different studies may use varying terms or regional boundaries, and there is no universally agreed-upon classification system. Thus, we compiled a list of documented dialects based on established sociolinguistics research. We then group these dialects into general categories according to shared phonological and morphological features.

% We begin by examining the varieties of dialects identified in the Najd region. Najd is a historical region of the Arabian Peninsula that encompasses most of central Saudi Arabia. It is generally bounded by the Hejaz region to the west, the Nafud desert in the north, the ad-Dahna desert in the east, and the Rub' al-Khali in the south, although its precise borders have shifted historically due to geographical and political factors \cite{britannica2024najd}. The Najd region is characterized by a number of dialectal varieties, each displaying distinctive features that set them apart from those spoken elsewhere in the Arabian Peninsula. In general,  several sub-dialects are identified within the broader category of Najdi dialect \cite{ingham1994najdi}:


% \begin{itemize}
%   \item \textbf{Central Najdi}: Spoken in the heart of the Najd region, including by central Bedouin tribes and groups such as the ʿAnizah in the Syrian desert.
%   \item \textbf{Northern Najdi}: Associated with the Jabal Shammar area and the Shammar tribes found in northern Najd. 
%   \item \textbf{Mixed Northern-Central}: Characteristic of the Qassim region and tribes like the Dhafir, showing features of both northern and central varieties.
%   \item \textbf{Southern Najdi}: Found in the southern areas such as Najran, and among tribes like the Ghatan, Al Murrah, and Ajman in the eastern and southern parts of the country.
% \end{itemize}

% Another major part of Saudi Arabia is the Hijaz region, which is a historically significant region in western Saudi Arabia that stretches along the Red Sea coast and encompasses the major cities of Mecca, Medina, Jeddah, Yanbu, and Taif, as well as the surrounding tribal areas \cite{destinationksa_hejaz}. Linguistically, the region is far from homogenous. The so-called ``Hijazi dialect'' is not a single variety but rather a collection of dialects that can be grouped into two main categories \cite{sambas2016hijazi}:

% \begin{itemize}
%   \item \textbf{Urban Hijazi}: Spoken in the large cities of Mecca, Medina, Jeddah, Taif, and Yanbu. These cities have long attracted Arabs and Muslims, whether to live in proximity to the holy sanctuaries of Mecca and Medina or for economic and social opportunities, creating a speech variety shaped by both native residents and long-term settlers. This is the dialect that most people typically identify as ``Hijazi Arabic.''

%   \item \textbf{Tribal Hijazi}: Associated with the speech of Bedouin tribes inhabiting the broader Hijaz region. These dialects preserve Bedouin phonological and morphological features and are spoken by tribal groups whether in rural areas or, in some cases, within urban settlements.

% \end{itemize}

